Precise Object Sliding with Top Contact via Asymmetric Dual Limit Surfaces

In this paper, we discuss the mechanics and planning algorithms to slide an object on a horizontal planar surface via frictional patch contact made with its top surface. Here, we propose an asymmetric dual limit surface model to determine slip boundary conditions for both the top and bottom contact. With this model, we obtain a range of twists that can keep the object in sticking contact with the robot end-effector while slipping on the supporting plane. Based on these constraints, we derive a planning algorithm to slide objects with only top contact to arbitrary goal poses without slippage between end effector and the object. We validate the proposed model empirically and demonstrate its predictive accuracy on a variety of object geometries and motions. We also evaluate the planning algorithm over a variety of objects and goals demonstrate an orientation error improvement of 90\% when compared to methods naive to linear path planners.

==> subsections/Relatedworks_archived.tex <==
% Planar manipulation tasks are strongly affected by object dynamics and friction wrenches. In \citep{goyal1989planar}, Goyal defined limit surface as the boundary of set of all possible friction wrenches and gave a simplified ellipsoidal model to reduce computation complexity. This model based on Coulomb Friction Model. In the work of  \citep{howe1996practical}, different models for limit surface were proposed and compared.

The contact mechanics in a planar manipulation task is complex \citep{johnson1989normal}. \citep{howe1988sliding} studied the contact between robot finger and object at the initiation of slippage under both torsion and shear. In \citep{goyal1989planar}, Goyal defined limit surface as the boundary of set of all possible friction wrenches to characterize the friction between two surfaces. In the work of \citep{howe1996practical}, different models for limit surface were proposed and compared, and a simplified ellipsoidal model was proposed to reduce computation complexity. In \citep{xydas1999modeling}, modeling and experimental results are proposed to evaluate the relationship between the normal force and radius of contact for soft fingers. In \citep{shi2017dynamic} Shi et al. derived a model of the sliding dynamics based on the limit surface contact model at each fingertip. In this work we also used the ellipsoidal approximation of limit surface to model the friction behavior for each contact. Moreover, we extend these models to a multi-contact scenario.

Modeling, planning and control of planar pushing are widely studied in the past. A motion planning algorithm under the assumption that sticking interaction is maintained to find trajectories to target goals were introduced by Lynch and Mason\citep{lynch1996stable}. The work in \citep{yu2016more} did a comprehensive study in evaluating different friction models by pushing objects with different materials, shapes, contact locations, directions, velocity and accelerations. We choose the material for experiments based on this work.

The problem of planar manipulation with top contacts \citep{kao1992quasistatic,kao1993comparison,xue1994dexterous,9811686,ghazaei2020quasi,fakhari2019modeling,zhou2016convex} is less discussed than planar pushing problems than pushing. This kind of manipulation is usually called as dragging or sliding, in comparison with pushing, which relies on normal force on object sides. All these works also rely on a quasi-static analysis and Coulomb friction with limit surface modeling as well as soft contacts that allow moment transfer\citep{9811686}. 
The work in \citep{kao1992quasistatic} studied a generic manipulation problem with compliance and sliding.
In the subsequent studies \citep{kao1993comparison} and \citep{xue1994dexterous}, the mechanics of manipulating a business card with two sliding robot fingers on a frictionless table were analyzed. However, we cannot make such frictionless assumption when sliding a heavier object in reality.
The work in \citep{ghazaei2020quasi} derives a hybrid dynamical system, validated via simulations and experiments, to predict and control the motion of the object and the interaction forces providing conditions for sticking, slipping and pivoting. They also proposed a possible planning problem of finding trajectories to slide an object from an initial to a desired pose such that the contact between surfaces is maintained and the normal force is within desired limits.

The work in \citep{fakhari2019modeling} discussed the design of a controller to reduce the undesired slippage between top surface of object and robot finger, of an unknown object. This work is done only in simulation. These works all based on accurate force/torque control.
The work in \citep{9811686} includes a model free method for dragging an object to manipulate object with unknown dynamic and friction parameters. However, this works focused on planar translation, while not considering controlling rotation by sliding. 
The work in \citep{zhou2016convex} proposed a polynomial force-motion model for planar sliding with data-driven methods.

In the sliding problem we discuss in this paper, a path planning algorithm is proposed to get rid of slippage between end-effector and object under a specified normal force while sliding. This slippage-free planning algorithm aim to work not only for translation but also rotation, without force feedback along the path.


% For example, the work in \citep{ghazaei2020quasi} derives a hybrid dynamical system, validated via simulations and experiments, to predict and control the motion of the object and the interaction forces providing conditions for sticking, slipping and pivoting. 

==> subsections/experiments/data_processing.tex <==
We \todo{discuss this section with Xili}need to convert all raw data into points in form of limit surface. Considering that with isotropic friction assumption, $F_x$ and $F_y$ are equivalent, we will do a conversion to horizontal friction force $F_h = \sqrt{F_x^2+F_y^2}$. Then we can express wrenches in a dual-limit-cones plot, with their corresponding normal force.

With the object pose data along the whole path and raw F/T sensor data, we can calculate the wrench applied to the object in its own frame along the whole path. Considering the constant linear and angular velocity, we can assume the wrench applied to the object is constant.  At the beginning and the ending part of each path, the force is different because of the dynamics of the object, which is not in our assumptions. Thus after transformation, we will crop the beginning and ending data. Then we obtain the friction wrench for each path as the average of wrench respect to object frame.
Considering symmetric, all data is shown in quarter of dual-limit-cones.

% For all data from experiments, we will first do wrench transformation to the object frame. Here we assume the object always follows the finger because we don't have the object pose directly. At the beginning and the ending part of the measurement, the force is different because of the dynamics of the object, which is not in our assumptions. Thus after transformation, we will crop the beginning and ending data, then get the average horizontal force $F_h$ and normal torque $m_z$ for each single path.
% \begin{figure} 
% \centering
% \includegraphics[width=8cm]{figs/Picture17.png}
% \caption{Raw horizontal force measured from F/T sensor with same normal force with different poses}
% \label{fig:force_measured}
% \end{figure}

==> subsections/experiments/limit_surface_experiment.tex <==
The first experiment is to validate limit surface module, which is also used to validate the effectiveness of the experiment setup.
The normal force applied by the finger is set to be 8N, the diameter of the finger tip is 25 mm, the diameter of the object is 70.0mm. The mass of the object it 59.2g.
To validate limit surface model, we have to guarantee the object moves on the supporting plane, while not slipping with the finger. In dual-limit-surfaces model section, we showed that with bigger normal force, we are able to make the object follows the finger. 

Paths are designed with the following features:
\begin{enumerate}
\item For each single path, the linear and angular velocity are constant
\item For each single path, the start point is at the center of the supporting plane.
\end{enumerate}
The robot moves the finger above the object, then apply the normal force. When it is stable, the robot executes one of the designed paths, meanwhile measure the force torque data with sensor and record corresponding finger poses. After executing each path, robot moves the object back to the center of the supporting plane, and repeat the previous steps. Each path is executed for 3 times.



==> subsections/experiments/path_execution.tex <==
\begin{figure*} 
\centering
% \includegraphics[width=8cm]{figs/results/path_error.jpg}
% \includegraphics[width=16cm]{figs/results/path_error_histogram_1_4.png}
\includegraphics[width=18cm]{figs/results/path_error_histogram_1_6.jpg}
\caption{RMSE of pose at the goal poses with naive paths and planned paths with different normal force.}
\label{fig:path_error}
\end{figure*}

To evaluate the path planning algorithm, 
we measure the pose errors between the goal and achieved poses at the end of each path for both our proposed and naive planners. In all paths, we kept the end-effector move in the same horizontal plane. The physical parameters are fit to cases (c) or (d). We executed 162 paths with translation magnitudes ranging from 0.02 to 0.04 [M], rotation magnitudes from 0.5 to 0.9 [Rad], and normal forces from 3 to 5 [N]. These path parameters are chosen based on the size of supporting plane, size of the object and friction coefficients. The RMSE of relative pose errors at the end of both paths are shown in Table \ref{tab2} and in Fig. \ref{fig:path_error}. Considering that pose error caused by Apriltag has RMSE of 0.0008 [M] in position and 0.002 [Rad] in orientation, the translation error can be neglected. 
% (This part needs experiments, current numbers are just arbitrary number) 
We note that the planned path shows significant improvement in orientation error. 

\begin{table*}[h]
\begin{center}
\caption{Path execution results}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
\textbf{Object} & \textbf{Round} & \textbf{Square} & \textbf{Rectangle} & \textbf{Irregular} & \textbf{Triangle} & \textbf{Average}\\ \hline
Naive pos. RMSE/m & 0.0013  & 0.0014 & 0.0013 & 0.0020 & 0.0019 & 0.0016 \\ \hline
Naive ori. RMSE/rad & 0.1885 & 0.3354 & 0.1918 & 0.1646 & 0.1471 & 0.2055 \\ \hline
Planned pos. RMSE/m & 0.0009 & 0.0015 & 0.0013 & 0.0018 & 0.0019 & 0.0015 \\ \hline
Planned ori. RMSE/rad & 0.0071 & 0.0087 & 0.0072 & 0.0171 & 0.0176 & 0.0116 \\ \hline

\end{tabular}
\label{tab2}
\end{center}
\end{table*}

\begin{figure} 
    \centering
    \includegraphics[width=7.7cm]{figs/results/planned_vs_linear_path_3d.png}
    \caption{3D visualization of a pair of sample paths in configuration space. Both paths starts from [0,0,0] and ends at[0, -0.01, -0.7]. 3 axes represents \(x\), \(y\) and \(\theta\) of each trajectory. Blue and red curves are the end-effector and object trajectories with planned path, while green and orange ones are end-effector and object trajectories with naive path. %We assume that the end-effector trajectory matches the planned path.
    }
    \label{fig:path_sample_3d}
\end{figure}

\begin{figure*} [b]
    \centering
    \includegraphics[width=15cm]{figs/pictures/Final_result_4.jpg}
    \caption{visualization of the path of object starts from [0, 0, 0] and ends at[0.05, 0, -1.57]. In each column, the top shows the scheme of pose, the bottom show the pose in real scene. (a) shows the start and desired goal pose, (b) shows the planned path and corresponding sliding result, (c) shows the naive path and corresponding sliding result.}

    \label{fig:path_sample_real_sim}
\end{figure*}

Fig.~\ref{fig:path_sample_3d} shows example robot planned paths and corresponding object paths in configuration space for a given goal from both our approach and the naive planner. Here, the $(x,y)$ axes represent translations, and z axis represents rotation \(\theta\). The blue curve shows the end-effector path computed from our method and the red curve shows the corresponding realized object path. We note that the object closely follows the end-effector and reaches the desired goal. In contrast, the green curve is the linear naive end-effector path from the start pose to the goal, while the orange curve is the corresponding object trajectory. We highlight that the object fails to follow the end-effector with the naive linear path, where the deviation is especially pronounced in rotation. \textcolor{blue}{Fig.~\ref{fig:path_sample_real_sim} also shows a visualization of paths and results in both scheme and real experiments.}

\textcolor{blue}{We also noticed that the RMSE rotational of planned paths for irregular shape and triangle are higher than that for round, square and rectangle shapes. That could cause by the loss of rotational symmetry of 90 degree, and more nonuniform pressure distribution.}

% To better visualize the executed path, Fig. \ref{fig:path_sample_3d}
% % and Fig. \ref{fig:path_sample_majong} 
% shows one sample path. 
% In Fig. \ref{fig:path_sample_3d}, x axis represents translation in x direction, y axis represents translation in y direction, and z axis represents rotation \(\theta\). Two paths are shown in this figure, with the blue curve shows planned path for end-effector, the red curve shows the corresponding real path of the object.
% The green curve is the linear path from start pose to goal for the end-effector, while the orange curve is the corresponding trajectory. While executing the planned path, the object follows end-effector along the whole path. In comparison, the object fails to follow the end-effector with a naive linear path, especially in rotation.
% \todo{Figure 12 not completed, need to change style}

% \begin{figure} 
% \centering
% \includegraphics[width=8cm]{figs/results/planned_vs_linear_path_2d.jpg}
% \caption{2D visualization of a pair of sample paths. Both paths starts from [0,0,0] and ends at[0.001, -0.01, -0.7].}
% \label{fig:path_sample_2d}
% \end{figure}

==> subsections/mechanics/dual_limit_surfaces.tex <==
To develop the dual-limit surfaces model, consider Fig. \ref{fig:teaser_1}(b) where the end-effector is in contact with the top surface of the object while the object is also in contact with a supporting plane. Here, the supporting planes are perpendicular to the direction of gravity. For scenarios in which the end-effector’s center is aligned with the object center, and the end-effector has a symmetric geometry, we have two center-aligned contact surfaces. For each contact surface, we can plot a limit-surface corresponding to the normal force.

% The dual-limit surfaces model is developed from the limit surface model at scene shown in Fig. \ref{fig:teaser_1}(b). An end-effector is in contact with an flat object while the object is also in contact with a supporting plane. The supporting plane is perpendicular to gravity direction. In simplified scenarios in which the end-effector’s center is at the center of the object, and the end-effector has a symmetric geometry, we have two contact surfaces which are aligned at the center of each other. For each contact surface, we can plot a limit-surface corresponding to the normal force.

Let $N_e$ denote the normal force applied by the end-effector to the object, then the normal force between the object and supporting plane \(N_p\) is the sum of gravity force and the applied normal force:
\begin{equation*}
    N_p=mg+N_e
    \label{eqn:normal_plane}
\end{equation*}
For a choice of $N_e$ and physical parameters (mass, friction, and equivalence radii), we can plot the 2 limit-surfaces in the object wrench space, as shown in Fig. \ref{fig:slippage-free_twist_with_DLS}(a). With the quasi-static assumptions, considering force-torque balance on the x-y plane, we have:
\begin{equation*}
\vec{w_e}+\vec{w_p}=0
\label{eqn:balance_plane}
\end{equation*}
where \(\vec{w_e}\) is the wrench applied by the end-effector to the object projected to supporting plane contact frame, \(\vec{w_p}\) is the wrench applied from the supporting plane to the object.
\begin{figure} 
    \centering
    \includegraphics[width=8cm]{figs/schematic/Dual_limit_surfaces_feasible_wrenches_scheme_2.png}
    \caption{(a) Schematic of slippage-free twists on the dual-limit surfaces model. The blue ellipse represents the limit surface between the object and end-effector while the orange ellipse represents the limit surface between the object and the supporting plane. Wrenches on the \textcolor{red}{I dont see red in the figure:}red surface mean the object is moving on the supporting plane or is static. Wrenches on the green surface mean the object is \textcolor{red}{do you mean sticking? if yes, change staying:}staying on the supporting plane while the end-effector slips on the object or is static. Wrenches inside the green and red surfaces mean the object is static. All directions of slippage-free twists should be the collection of norm directions of all points on the green surface, as shown on panel (b).}
    \label{fig:slippage-free_twist_with_DLS}
\end{figure}
These two wrenches are equal in magnitude but opposite in direction, considering that both limit surfaces are symmetric to the origin point, we can use single point in this dual-limit-surfaces to represent this pair of friction wrenches.  
\begin{figure*} 
\centering
\includegraphics[width=170mm]{figs/schematic/DLS_4cases_2.png}

\caption{Schematic of dual-limit cones in 4 cases. The top row shows the schematics of dual-limit-cones, where red surfaces and curves represent the contact between end-effector and object, green ones represent the contact between object and its supporting plane. The bottom row shows the projections of dual-limit-cones on to F-T plane. Also, 2D dual-limit-surfaces with different normal forces are also shown in these figures. The slippage boundaries regardless of the normal forces are normal of limit surfaces at the boundary between green and red area. To be noticed, these boundaries composites with all intersection points for every 2D dual-limit-surfaces.}
\label{fig:dual_limit_surface_different_cases}
\end{figure*}


By definition, all frictional wrenches are either inside or on the limit-surface. Therefore, both \(\vec{w_e}\) and \(\vec{w_p}\) must be inside or on their respective limit surfaces. As a result, the frictional wrench should be inside or on the intersection of both limit-surfaces in Fig. \ref{fig:slippage-free_twist_with_DLS}(a).

\sout{While} \todo{This sentence is a bit hard to understand.} \sout{on-surface wrenches mean dynamic or static friction, in-surface wrenches mean static friction, we have 3 different cases: }
\textcolor{blue}{According to the previous derivation, there are 3 cases:} i) \todo{what is static? the object? Lets specify}\textcolor{blue}{neither the object or the end-effector moves} (inside both green and red surfaces), ii) the object slips on the supporting plane while sticking to the end-effector (on green surface), and iii) the object sticks to the supporting plane while the end-effector slips on the object (on red surface). 


With the assumption of symmetric and homogeneous friction properties, planar translation along \(F_x\) and \(F_y\) axes are equivalent. Thus, we can reduce the dual-limit surfaces at a certain normal force in to 2D space, with one axis representing friction force, and the other representing friction torque. Next, we add the axis of normal force \(N_p\) to visualize how dual-limit-surfaces change with respect to the normal force. We call this construct the dual-limit cones, visualized in Fig. \ref{fig:dual_limit_surface_different_cases}. This model extends the work in \citep{9811686}, as the cross-section along \(T\)-\(N_p\) plane is the Friction Cone Diagram with pure translation. Cross-sections at certain \(N_p\) parallel to T-F plane represent dual-limit-surfaces at certain normal force. The two cones are shifted along the \(N_p\) axis by the magnitude of the gravity force acting on the object. The projection of the intersection of the two cone limit-surfaces on the F-T plane represents the boundary of slippage of all normal forces, and we can divide this boundary of slippage into 4 cases, shown in Fig. \ref{fig:dual_limit_surface_different_cases}. These four cases are determined by the following parameters:
\begin{equation*}
p_T = \mu_e r_e - \mu_p r_p, \quad p_F = \mu_e - \mu_p
\end{equation*}
where \(p_T\) and \(p_F\) are the differences between the slopes of the two cones along the \(T\) and \(F\) axis, respectively.
Four cases are shown in four columns. In each column, the top row is the condition, the middle is the 3D visualization of the dual-limit cones, and the bottom is their projection on the F-T plane. This projection shows the boundary of slippage of certain geometry and friction parameters, regardless of the normal force \(N_e\). The robot is able to maintain sticking contact with the object by imparting wrenches in the green zone. 

\textcolor{blue}{In the following section, we will not discuss case (a) as the object cannot move no matter what wrench is applied. When the normal force is greater than \({N_e}_{slip}\), in case (b),  }

\sout{We will discuss case (c) and (d) in the following motion planning section, as no motion could be planned for case (a), and we will not face case (b) as the end-effector's diameter is smaller than the object, }\todo{instead of this sentence (from though it could happen) can you instead explain how the analysis would change?}\sout{though it could happen if the end-effector contact patch has a larger diameter than supporting plane contact patch. }

% \todo{the following parts can be deleted if run out of space, I think }

Changing normal force will change the relative size of these 2 limit surfaces, as it will change the ratio between normal forces applied through each contact: %on 2 limit surfaces. 
\begin{equation*}
    R=\frac{N_e}{N_e+mg}
    \label{eqn:ratio}
\end{equation*}
With normal force increasing, the ratio $R$ increases, which will result in a taller intersection between the 2 limit surfaces. It's easy to know that the upper limit of \(R=1\). When the normal force \(N_e\) is smaller than:
\begin{equation*}
    {N_e}_{slip}=\frac{\mu_pmg}{\mu_e-\mu_p}
    \label{eqn:force_slip}
\end{equation*}
% where $\mu_p$, $\mu_f$ are the friction coefficient of object-supporting plane and object-end-effector.
\todo{what will reduce?}it will reduce to single limit surface between the object and end-effector, as there is no intersection between these 2 limit surfaces, which means the end-effector will always slip on the object.

In case (d), increasing the normal force may result in the limit surface of the object and supporting plane to lie entirely inside the limit surface of the end-effector and object, which means the object will always follow the end-effector. The boundary normal force will be:

\begin{equation*}
    {N_e}_{stick}=\frac{r_p\mu_pmg}{r_f\mu_f-r_p\mu_p}
    \label{eqn:force_boundary}
\end{equation*}
when the normal force \(N_e\) is bigger than \({N_e}_{stick}\), the object will always stick to the end-effector. 



